MAPTree: Beating "Optimal" Decision Trees with Bayesian Decision Trees

Decision trees remain one of the most popular machine learning models today, largely due to their out-of-the-box performance and interpretability. In this work, we present a Bayesian approach to decision tree induction via maximum a posteriori inference of a posterior distribution over trees. We first demonstrate a connection between maximum a posteriori inference of decision trees and AND/OR search. Using this connection, we propose an AND/OR search algorithm, dubbed MAPTree, which is able to recover the maximum a posteriori tree. Lastly, we demonstrate the empirical performance of the maximum a posteriori tree both on synthetic data and in real world settings. On 16 real world datasets, MAPTree either outperforms baselines or demonstrates comparable performance but with much smaller trees. On a synthetic dataset, MAPTree also demonstrates greater robustness to noise and better generalization than existing approaches. Finally, MAPTree recovers the maxiumum a posteriori tree faster than existing sampling approaches and, in contrast with those algorithms, is able to provide a certificate of optimality. The code for our experiments is available at https://github.com/ThrunGroup/maptree.

==> old.tex <==
\textbf{class ORNode:}\\

\texttt{ \# pre-defined} \\
\texttt{depth: int = 0} \\ 
\texttt{stop\_child: TerminalNode} \\
\texttt{split\_children: List[ANDNode]} \\
\texttt{parents: List[ANDNode]} \\ 

\texttt{ \# updated by MAPTree} \\
\texttt{expanded: bool = False} \\
\texttt{lb: float = 0} \\
\texttt{ub: float = $\infty$} \\
\texttt{lb\_ptr: ANDNode} \\
\texttt{ub\_ptr: ANDNode} \\

\textbf{class ANDNode:}\\

\texttt{ \# pre-defined} \\
\texttt{parent: ORNode} \\ 
\texttt{split\_on: int}\\
\texttt{left: ORNode}\\
\texttt{right: ORNode}\\

\texttt{ \# updated by MAPTree} \\
\texttt{lb: float = 0} \\
\texttt{ub: float = $\infty$} \\


Random equations:
\begin{align}
    P(\mathcal{Y} | \mathcal{X} , T) &= \prod_i P(y_i | x_i, T) \\
    &= \prod_i p_{l_i}(y_i)
\end{align}

More equations:

\begin{align}
    p_{l_i}(y_i) &= \int_{\theta_{l_i} = 0}^{1} p(y_i | \theta_{l_i}) p(\theta_{l_i}) d\theta_{l_i} \\
    &= \int_{\theta_{l_i} = 0}^{1} \theta_{l_i}^{y_i} (1-\theta_{l_i})^{1-y_i} p(\theta_{l_i}) d\theta_{l_i} \\ 
    &= \int_{\theta_{l_i} = 0}^{1} \theta_{l_i}^{y_i} (1-\theta_{l_i})^{1-y_i} \frac{\theta_{l_i}^{\rho_1 -1} (1-\theta_{l_i})^{\rho_0 - 1}}{B(\rho_0, \rho_1)} d\theta_{l_i}  \\  % TODO: Check these exponents are correct
    &= \frac{B(\rho_0 + (1-y_i), \rho_1 + y_i)}{B(\rho_0, \rho_1)}
\end{align}


\begin{proof}

By the independence assumption, we may write
\begin{equation}
    \Pr[Y | X, T] = \prod_{i = 1}^n \Pr[y_i | x_i, T].
\end{equation}

Furthermore, by grouping the terms in the product on the right hand side by leaf node, we may write

\begin{align}
    \prod_{i = 1}^n \Pr[y_i | x_i, T] &= \prod_{j = 1}^{b(T)} \prod_{r=1}^{n_j} \int_{\theta} \Pr[y_i | \theta_j, x_i, T] \Pr[\theta_j] d\theta_j \\
    &= \prod_{j = 1}^{b(T)} \prod_{r=1}^{n_j} \int_{\theta} \Pr[y_i | \theta_j] \Pr[\theta_j] d\theta_j
\end{align}

where $n_j$ is the number of datapoints in leaf $j$ of tree $T$ and since $Pr[y_i | \theta_j, x_i, T] = Pr[y_i | \theta_j]$ as the prediction $y_i$ only depends on the parameter $\theta_j$. 
Furthermore, 

\begin{align}
    \prod_{r=1}^{n_j} \int_{\theta_j} \Pr[y_r | \theta_j] \Pr[\theta_j]d\theta_j &= \int_{\theta} \prod_{r=1}^{n_j}  \Pr[y_r | \theta_j] \Pr[\theta_j]d\theta_j \\
    &= \frac{B(n_j + \alpha)}{B(\alpha)}
\end{align}

for each $j$, where we used the fact that $ \Pr[\theta_j] \propto \theta_{j, 1}^{\alpha_1 - 1} \ldots \theta_{j,C}^{\alpha_C - 1}$ and results from \cite{denisonBayesianCARTAlgorithm1998b}. Thus 

\begin{equation}
    \Pr[Y | X, T] = \prod_{j=1}^{b(T)}  \frac{B(n_j + \alpha)}{B(\alpha)}
\end{equation}

as desired.
\end{proof}


% With this notation, we state the following theorem:
% \begin{theorem}
%     \label{thm:y_given_xt}
%     Assume that labels are drawn independently from their respective distributions conditioned on $T$ and $\Theta$.  
%     Further, assume a Beta prior $\text{Beta}(\rho^0, \rho^1)$ for each parameter $\theta_1, \dots, \theta_{b(T)}$.
%     Then the likelihood for dataset labels $Y$ given the predictors $X$ and binary tree $T$ is
    
%     \begin{equation}
%     \label{eqn:likelihood}
%         \Pr[Y \mid X, T] = \prod_{j=1}^{b(T)} \frac{B(n_j^0 + \rho^0, n^1_j + \rho^1)}{B(\rho^0, \rho^1)}
%     \end{equation}
    
%     where $n^0_j$ is the number of $0$-labelled points in the $j$th terminal node, $n^1_j$ is the number of $1$-labelled points in the $j$th terminal node, and $B$ is the beta function.
% \end{theorem}

% Theorem \ref{thm:y_given_xt} allows us to compute the the likelihood of labels $Y$ occurring for data $X$ under a given tree structure $T$ and choice of leaf node probability distributions $f(y | \theta_1), \dots, f(y | \theta_{b(T)})$ where each $f$ is a Dirichlet distribution parameterized by its corresponding $\theta$.
% For example, with the tree $T$ and points in Figure \ref{fig:decision-tree}, assuming a uniform prior where $\alpha = (1, 1)$, the conditional likelihood $\Pr[Y | X, T]$ of generating the provided labels is $\frac{B(2, 3)B(1, 3)B(4, 2)}{B(1, 1)^3}$.

% Our goal, however, is to sample trees from the posterior $\Pr [T \mid X, Y]$. To do so, we must also choose a prior across trees $\Pr[T | X]$.
% As noted in previous work \cite{buntineLearningClassificationTrees1992}, the support of this distribution will depend on our data $X$ due to the following natural constraints, which we call the Tree Constraints:
% \begin{enumerate}
% \label{lst:constraints}
%     \item the bounding boxes of nodes in $T$ must be nonempty, and
%     \item any splits on a node which result in the same two divided bounding boxes are considered equivalent.
% \end{enumerate}
% These constraints significantly reduce the considered space of trees considered.
% In particular, the number of possible trees is finite.

% We use a basic prior mentioned in previous work \cite{denisonBayesianCARTAlgorithm1998b,chipmanBayesianCARTModel1998c} which scales exponentially with the number of terminal nodes in the tree. 
% This choice of prior biases the tree search towards smaller trees:
% \begin{equation}
% \label{eqn:prior}
%     \Pr[T \mid X] \propto \phi^{-b(T)}
% \end{equation}

% \begin{theorem}
% \label{thm:posterior}
% The posterior over trees resulting from the likelihood in Equation \eqref{eqn:likelihood} and prior in Equation \eqref{eqn:prior} is:
% \begin{equation}
%     \Pr[T \mid X, Y] \propto \left( \prod_{k=1}^{b(T)} \frac{B(n_k + \alpha)}{B(\alpha)} \right) \left( \phi^{-b(T)} \right)
% \end{equation}
% \end{theorem}

% \begin{proof}
% A straightforward application of Bayes' rule yields

% \begin{align}
%     \Pr[T \mid X, Y] & \propto \Pr[Y \mid X, T]\Pr[T \mid X] \\
%     &= \left( \prod_{k=1}^{b(T)} \frac{B(n_k + \alpha)}{B(\alpha)} \right) \left( \phi^{-b(T)} \right)
% \end{align}
    
% \end{proof}

% Theorem \ref{thm:posterior} provides us with a posterior for the trees given the data.
% In later sections, we will define a method of sampling trees according to this posterior.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EXPAND NODE
% \begin{algorithm}[tb]
% \caption{expandNode}
% \label{alg:expandNode}
% \textbf{Input}: ORNode $o$ \\
% \begin{algorithmic}[1] %[1] enables line numbers

% \STATE $d = o.\text{depth}$
% \STATE $\mathcal{F} =$ findSplittableFeatures($\mathcal{X}_o, \mathcal{Y}_o)$
%     \FORALL{$f \in \mathcal{F}$}
%         \STATE Create ANDNode $a_f$ with $a_f.split\_on = f$ and $a_f.parent = o$
%         \STATE split\_prob = $\log p_\text{split}(d) - \logF$
%         \STATE $a_f.lb = a_f.Left.lb + a_f.Right.lb + $ split\_prob
%         \STATE $a_f.ub = a_f.Left.ub + a_f.Right.ub + $ split\_prob
%         \STATE $a_f.Left =$ createNode($d$, $\mathcal{X}_{o, f, l}$, $\mathcal{Y}_{o, f, l}$)
%         \STATE $a_f.Right = $ createNode($d$, $\mathcal{X}_{o, f, r}$, $\mathcal{Y}_{o, f, r}$)
%         \STATE $o.\texttt{children}.\texttt{append}(a_f)$
%     \ENDFOR
% \STATE o.expanded = True
% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BUILD NODE FUNCTION
% \begin{algorithm}[tb]
% \caption{createNode}

% \textbf{Input}: Depth $d$, Dataset $\mathcal{X}_o$ with labels $\mathcal{Y}_o$
% \textbf{Output}: ORNode $o$
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE leaf\_value = $\log p_\text{leaf}(d, \mathcal{X}_o, \mathcal{Y}_o)$
% \STATE Create terminal ORNode $o_t$ with depth $d$ and upper and lower bounds both equal to leaf\_value, expanded = True
% \STATE Create ORNode $o$ with depth $d$ and upper bound $h(d, \mathcal{X}_o, \mathcal{Y}_o)$ and lower bound to leaf\_value
% \STATE $o.children = \{ o_t\}$

% \STATE Create ORNode $o_{f, r}$ with depth $o.d + 1$ and lower bound $h(o.d + 1, \mathcal{X}_o_{f, r}, \mathcal{Y}o_{f, r})$ and upper bound $p_\text{stop}(d)$
% \STATE Create ANDNode $a_f$ with $a_f.split\_on = f$ and $a_f.parent = o$
% \STATE $o.\texttt{children}.\texttt{append}(a_f)$
% \STATE Create ORNode $o_{f, l}$ with depth $o.d + 1$ and lower bound $h(o.d + 1, \mathcal{X}_o_{f, l}, \mathcal{Y}o_{f, l})$ and upper bound $p_\text{stop}(d)$
% \STATE Create ORNode corresponding to terminating at $o$ 
% \STATE $a_f.Left = o_{f, l}$
% \STATE Create ORNode $o_{f, r}$ with depth $o.d + 1$ and lower bound $h(o.d + 1, \mathcal{X}_o_{f, r}, \mathcal{Y}o_{f, r})$ and upper bound $p_\text{stop}(d)$
% \STATE $a_f.Right = o_{f, r}$

% \RETURN $o$
% \end{algorithmic}
% \end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Find Splittable Features

% \begin{algorithm}[tb]
% \caption{\texttt{findSplittableFeatures}}
% \label{alg:findSplittableFeatures}
% \textbf{Input}: ORNode $o$, dataset $\mathcal{X}_o$ with $F$ features, and labels $\mathcal{Y}_o$\\
% \textbf{Output}: $\mathcal{F} \subset \{1, \ldots, F\}$, a subset of splittable features\\
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE $\mathcal{F} = \emptyset$
% \FORALL{$f \in 1, \ldots F$}
%     \IF{$\exists$ $x_i$ s.t. $(x_i)_f = 0$ and $\exists$ $x_j$ s.t. $(x_j)_f = 1$}
%         \STATE $\mathcal{F} = \mathcal{F} \cup f$
%     \ENDIF
% \ENDFOR
% \RETURN $\mathcal{F}$
% \end{algorithmic}
% \end{algorithm}



    
    % \begin{enumerate}
    %     \item Create a root OR node $r$ with associated dataset $(\mathcal{X}_u, \mathcal{Y})_u$. Mark $r$ as ``unexpanded.''
    %     \item While there is an unexpanded OR node $o$ with associated dataset $(\mathcal{X}_o, \mathcal{Y}_o)$:
    %     \item Create a terminal node $u_t$ and create an edge from $u$ to $u_t$ with cost $p_\text{stop}(d)$
    %     \item For each feature that has distinct values in $(\mathcal{X}_u, \mathcal{Y})_u$ Create an AND Node
    %     \item Create an OR node
    %     \item Mark $u$ as expanded
    % \end{enumerate}

    % Note that the definition above is recursive. 

    In the binary classification setting, we are given a dataset $\mathcal{X}, \mathcal{Y}$ and our goal is to learn a tree model that can accurate predict $y_i$ given $x_i$.


    

%We focus on binary datasets and binary classification for simplicity; any dataset can be binarized

%Constructive Tree Prior \mo{cite}



% \begin{equation}
%     p_\text{stop}(d, \mathcal{X}_o) = 
%       \begin{cases}
%       1, & \text{if}\ \texttt{findSplittableFeatures($\mathcal{X}_o$)} = \emptyset \\
%       1 - p_\text{split}(d), & \text{otherwise}
%     \end{cases}
% \end{equation}



%%%%%%%%%%%%%%%%%%%%% Random equations


% So we can convert the equation to 

% \begin{align}
%     P(\mathcal{Y} | \mathcal{X} , T) &= \prod_i p_{l_i}(y_i) \\
%     &= \prod_{j = 1}^{b(T)} \frac{B(\rho_0 + n_0(j), \rho_1 + n_1(j))}{B(\rho_0, \rho_1)^{n(j)}}
% \end{align}

% \mo{n is also a function of the data, so instead just index it instead of making it a function. So $n_j$ is the number of datapoints in leaf $j$}

% where the index $j$ runs over the leaves in $T$. Then

% Single leaf log likelihood of data on a single leaf

% \begin{align}
%      p_{l_i}(y_i) &= \frac{B(\rho_0 + n^0(l_i), \rho_1 + n^1(l_i))}{B(\rho_0, \rho_1)^{n(l_i)}}
% \end{align}

% \mo{Cite constructive tree prior}

% Total log probability of terminal node is 

% \begin{align}
%     p_\text{leaf}(d, \mathcal{X}_\text{leaf}, \mathcal{Y}_\text{leaf}) &= \frac{B(\rho_0 + n^0(\mathcal{Y_\text{leaf}}), \rho_1 + n^1(\mathcal{Y_\text{leaf}}))}{B(\rho_0, \rho_1)^{n(\mathcal{Y_\text{leaf}})}} \\
%     &\times p_\text{stop}(d, \mathcal{X}_\text{leaf})
% \end{align}

% $n$ should be a function of $\mathcal{Y}$.

% Our heuristic is a tree stump that perfecdtly classifies all the data. The heuristic is then, from the above equation, 

